Learning Disentangled Representations for Natural Language Definitions

Disentangling the encodings of neural models is a fundamental aspect for improving interpretability, semantic control and downstream task performance in Natural Language Processing. Currently, most disentanglement methods are unsupervised or rely on synthetic datasets with known generative factors. We argue that recurrent syntactic and semantic regularities in textual data can be used to provide the models with both structural biases and generative factors. We leverage the semantic structures present in a representative and semantically dense category of sentence types, definitional sentences, for training a Variational Autoencoder to learn disentangled representations. Our experimental results show that the proposed model outperforms unsupervised baselines on several qualitative and quantitative benchmarks for disentanglement, and it also improves the results in the downstream task of definition modeling.

==> tables/generative_factors.tex <==
\begin{table}[h]
    \scriptsize
    \setlength\tabcolsep{3.5pt}
    \centering
    \begin{tabular}{llllllll}
        \hline \hline
        \multicolumn{8}{l}{GF1} \\
        Super.   & Quality & Event    & Loc.    & Mod.   & Stat. & Acc.   & \\
        ST       & DQ      & DE       & EL, OL  & QM, ET & P, AF & AD, AQ & \\ \hline
        \multicolumn{5}{l}{GF2} & & & \\
        Super.   & Main    & Mod E.   & Mod Q   & Acc.   &       &        & \\
        ST       & DQ,DE   & EL, ET   & QM,P,AF & AD,AQ  &       &        & \\ \hline
        \multicolumn{4}{l}{GF3} & & & & \\
        Quality  & Event   & Loc.     & Stat.   &        &       &        & \\
        DQ,QM,AQ & DE,ET   & EL,OL    & P,AF,AD &        &       &        & \\ \hline
        \multicolumn{4}{l}{GF4} & & & & \\
        Main     & Mod E   & Mod Q    & Acc.    &        &       &        & \\
        DQ,DE    & EL, ET  & QM,P,AF, & AD,AQ   &        &       &        & \\
        \hline \hline
    \end{tabular}
    \caption{Generative factors and their values.} \label{tab:gen_factors}
\end{table}



==> tables/wikipedia_all.tex <==
\begin{table*}[ht!]
    \centering
    \scriptsize
    %\resizebox{.95\columnwidth}{!}
    \begin{tabular}{ll|c|c|c|c|}
\cline{3-6}
                                       & \textbf{}               & \multicolumn{4}{c|}{\textbf{Groupings}}                                                                                                                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{\textbf{Metrics}} & \textbf{Experiments}    & \begin{tabular}[c]{@{}c@{}}1. Semantic\\ w/ supertype\end{tabular} & \begin{tabular}[c]{@{}c@{}}2. Syntactic\\ w/ supertype\end{tabular} & \begin{tabular}[c]{@{}c@{}}3. Semantic\\ w/o supertype\end{tabular} & \begin{tabular}[c]{@{}c@{}}4. Syntactic\\ w/o supertype\end{tabular} \\ \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & 53.8\% &                      60.5\% &                      49.7\% &                       66.0\%                                                               \\ \cline{2-6}
\multicolumn{1}{|l|}{$z_{diff}~acc.~\uparrow$}  & 2. Joint DSR loss       & 56.7\% &                      65.7\% &                      \textbf{57.0\%} &                       72.7\%                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & \textbf{59.8\%} &                      \textbf{71.4\%} &                      52.9\% &                       \textbf{74.8\%}                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  \textbf{29.5\%} &                      41.6\% &                      \textbf{40.5\%} &                       47.6\%                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$z_{min\_var}~err.~\downarrow$}       & 2. Joint DSR loss       &  29.9\% &                      \textbf{38.6\%} &                      42.6\% &                       \textbf{43.3\%}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  29.9\% &                      \textbf{38.6\%} &                      42.6\% &                       \textbf{43.3\%}                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  \textbf{0.052} &                      \textbf{0.050} &                      0.037 &                       \textbf{0.047}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$MIG~\uparrow$}              & 2. Joint DSR loss       &  0.043 &                      0.043 &                      0.040 &                       0.039                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  0.040 &                      0.031 &                      \textbf{0.043} &                       0.034                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  0.828 &                      \textbf{0.825} &                      \textbf{0.662} &                       \textbf{0.769}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$Modularity~\uparrow$}       & 2. Joint DSR loss       &  0.817 &                      0.807 &                      0.615 &                       0.743                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  \textbf{0.839} &                      0.799 &                      0.656 &                       0.733                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & 0.559 &                      0.525 &                      0.551 &                       0.546                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$Explicitness~\uparrow$}     & 2. Joint DSR loss       & 0.567 &                      0.546 &                      0.576 &                       0.538                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & \textbf{0.602} &                      \textbf{0.578} &                      \textbf{0.624} &                       \textbf{0.595}                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  0.006 &                      \textbf{0.010} &                      0.002 &                       0.010                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$Disentang. Score~\uparrow$} & 2. Joint DSR loss       &  \textbf{0.007} &                      0.009 &                      0.002 &                       \textbf{0.011}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  0.005 &                      0.007 &                      0.002 &                       0.006                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  \textbf{0.008} &                      \textbf{0.010} &                      \textbf{0.003} &                       0.008                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$Completeness~\uparrow$}     & 2. Joint DSR loss       &  \textbf{0.008} &                      \textbf{0.010} &                      \textbf{0.003} &                       \textbf{0.009}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  0.004 &                      0.005 &                      0.002 &                       0.003                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  0.417 &                      0.426 &                      \textbf{0.304} &                       0.353                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$Informativeness~\downarrow$}  & 2. Joint DSR loss       &  \textbf{0.413} &                      \textbf{0.422} &                      0.306 &                       0.350                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  0.417 &                      \textbf{0.422} &                      0.315 &                       \textbf{0.341}                                                                \\ \hline
\end{tabular}

    \caption{Wikipedia dataset - Impact of the DSR categorical biases: reconstruction. The arrow next to each metric indicates the direction of better disentanglement.}
    \label{tab:reconstr_impact_wkp}
\end{table*}


==> tables/wikipedia_by_exp.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{|l|c|c|c|}
        \hline
        \textbf{Metric} &      1. VAE reconst. &      2. Joint DSR loss &      3. cVAE ($token | DSR$) \\
        \hline
        $z_{diff}~acc.~\uparrow$       & 57.5\% &              63.0\% &                    \textbf{64.7\%} \\ \hline
        $z_{min\_var}~err.~\downarrow$   & 39.8\% &              \textbf{38.6\%} &                    42.0\% \\ \hline
        $MIG~\uparrow$                   &  \textbf{0.046} &              0.041 &                    0.037 \\ \hline
        $Modularity~\uparrow$            &  \textbf{0.771} &              0.745 &                    0.757 \\ \hline
        $Explicitness~\uparrow$          &  0.545 &              0.557 &                    \textbf{0.600} \\ \hline
        $Disentanglement Score~\uparrow$ &  \textbf{0.007} &              \textbf{0.007} &                    0.005 \\ \hline
        $Completeness Score~\uparrow$    &  \textbf{0.007} &              \textbf{0.007} &                    0.004 \\ \hline
        $Informativeness Score~\downarrow$ &  0.375 &              \textbf{0.373} &                    0.374 \\ \hline
    \end{tabular}

    \caption{Wikipedia dataset - Mean impact of the DSR categorical biases by model architecture.}
    \label{tab:aggr_model_impact_wkp}
\end{table*}


==> tables/wikipedia_by_group.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        \textbf{Metric} &      \begin{tabular}[c]{@{}c@{}}1.  Semantic\\ w/ supertype\end{tabular} &      \begin{tabular}[c]{@{}c@{}}2. Syntactic\\ w/ supertype\end{tabular} &      \begin{tabular}[c]{@{}c@{}}3. Semantic\\ w/o supertype\end{tabular} &      \begin{tabular}[c]{@{}c@{}}4. Syntactic\\ w/o supertype\end{tabular} \\
        \hline
        $z_{diff}~acc.~\uparrow$       & 56.8\% &                      65.9\% &                      53.2\% &                       \textbf{71.1\%} \\ \hline
        $z_{min\_var}~err.~\downarrow$   & \textbf{30.3\%} &                      41.7\% &                      40.8\% &                       47.7\% \\ \hline
        $MIG~\uparrow$                   &  \textbf{0.045} &                      0.041 &                      0.040 &                       0.040 \\ \hline
        $Modularity~\uparrow$            &  \textbf{0.828} &                      0.810 &                      0.644 &                       0.749 \\ \hline
        $Explicitness~\uparrow$          &  0.576 &                      0.550 &                      \textbf{0.584} &                       0.559 \\ \hline
        $Disentanglement Score~\uparrow$ &  0.006 &                      \textbf{0.009} &                      0.002 &                       \textbf{0.009} \\ \hline
        $Completeness Score~\uparrow$    &  0.007 &                      \textbf{0.008} &                      0.003 &                       0.007 \\ \hline
        $Informativeness Score~\downarrow$ &  0.416 &                      0.423 &                      \textbf{0.308} &                       0.348 \\ \hline
    \end{tabular}

    \caption{Wikipedia dataset - Mean impact of the DSR categorical biases by generative factor grouping.}
    \label{tab:aggr_grouping_impact_wkp}
\end{table*}


==> tables/wiktionary_all.tex <==
\begin{table*}[ht!]
    \centering
    \scriptsize
    %\resizebox{.95\columnwidth}{!}
    \begin{tabular}{ll|c|c|c|c|}
\cline{3-6}
                                       & \textbf{}               & \multicolumn{4}{c|}{\textbf{Groupings}}                                                                                                                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{\textbf{Metrics}} & \textbf{Experiments}    & \begin{tabular}[c]{@{}c@{}}1. Semantic\\ w/ supertype\end{tabular} & \begin{tabular}[c]{@{}c@{}}2. Syntactic\\ w/ supertype\end{tabular} & \begin{tabular}[c]{@{}c@{}}3. Semantic\\ w/o supertype\end{tabular} & \begin{tabular}[c]{@{}c@{}}4. Syntactic\\ w/o supertype\end{tabular} \\ \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & 56.4\% &                      60.8\% &                      64.9\% &                       56.7\%                                                               \\ \cline{2-6}
\multicolumn{1}{|l|}{$z_{diff}~acc.~\uparrow$}  & 2. Joint DSR loss       & 57.9\% &                      62.2\% &                      \textbf{69.6\%} &                       58.0\%                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & \textbf{59.0}\% &                      \textbf{66.8\%} &                      65.2\% &                       \textbf{63.0}\%                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  \textbf{31.9\%} &                      \textbf{42.3\%} &                      \textbf{44.8\%} &                       \textbf{41.0\%}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$z_{min\_var}~err.~\downarrow$}       & 2. Joint DSR loss       &  \textbf{31.9\%} &                      \textbf{42.3\%} &                      \textbf{44.8\%} &                       \textbf{41.0\%}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  32.4\% &                      44.7\% &                      45.9\% &                       49.0\%                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  \textbf{0.114} &                      \textbf{0.106} &                      \textbf{0.100} &                       \textbf{0.129}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$MIG~\uparrow$}              & 2. Joint DSR loss       &  0.095 &                      0.090 &                      0.088 &                       0.107                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  0.063 &                      0.068 &                      0.050 &                       0.078                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  0.341 &                      \textbf{0.730} &                      0.427 &                       \textbf{0.640}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$Modularity~\uparrow$}       & 2. Joint DSR loss       &  0.053 &                      0.726 &                      0.284 &                       0.634                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  \textbf{0.689} &                      0.686 &                      \textbf{0.560} &                       0.581                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & 0.600 &                      0.551 &                      0.627 &                       0.559                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$Explicitness~\uparrow$}     & 2. Joint DSR loss       & 0.608 &                      0.560 &                      0.640 &                       0.566                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & \textbf{0.629} &                      \textbf{0.585} &                      \textbf{0.649} &                       \textbf{0.602}                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  0.011 &                      0.016 &                      0.008 &                       \textbf{0.021}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$Disentang. Score~\uparrow$} & 2. Joint DSR loss       &  0.009 &                      0.012 &                      0.006 &                       0.017                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & \textbf{0.012} &                      \textbf{0.016} &                      \textbf{0.009} &                       0.016                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  0.011 &                      \textbf{0.015} &                      \textbf{0.010} &                       \textbf{0.018}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$Completeness~\uparrow$}     & 2. Joint DSR loss       &  \textbf{0.012} &                      0.013 &                      \textbf{0.010} &                       0.016                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  0.010 &                      0.013 &                      0.008 &                       0.013                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &  \textbf{0.388} &                      0.428 &                      0.354 &                       0.339                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$Informativeness~\downarrow$}  & 2. Joint DSR loss       &  \textbf{0.388} &                      \textbf{0.425} &                      \textbf{0.349} &                       \textbf{0.331}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) &  0.399 &                      0.434 &                      0.367 &                       0.341                                                                \\ \hline
\end{tabular}

    \caption{Wiktionary dataset - Impact of the DSR categorical biases: reconstruction. The arrow next to each metric indicates the direction of better disentanglement.}
    \label{tab:reconstr_impact_wkt}
\end{table*}


==> tables/wiktionary_by_exp.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{|l|c|c|c|}
        \hline
        \textbf{Metric} &      1. VAE reconst. &      2. Joint DSR loss &      3. cVAE ($token | DSR$) \\
        \hline
        $z_{diff}~acc.~\uparrow$       & 59.7\% &              61.9\% &                    \textbf{63.5\%} \\ \hline
        $z_{min\_var}~err.~\downarrow$   & 40.0\% &              \textbf{38.5\%} &                    43.0\% \\ \hline
        $MIG~\uparrow$                   &  \textbf{0.112} &              0.095 &                    0.065 \\ \hline
        $Modularity~\uparrow$            &  0.535 &              0.424 &                    \textbf{0.629} \\ \hline
        $Explicitness~\uparrow$          &  0.584 &              0.593 &                    \textbf{0.616} \\ \hline
        $Disentanglement Score~\uparrow$ &  \textbf{0.014} &              0.011 &                    0.013 \\ \hline
        $Completeness Score~\uparrow$    &  \textbf{0.013} &              \textbf{0.013} &                    0.011 \\ \hline
        $Informativeness Score~\downarrow$ &  0.377 &              \textbf{0.373} &                    0.385 \\ \hline
    \end{tabular}

    \caption{Wiktionary dataset - Mean impact of the DSR categorical biases by model architecture.}
    \label{tab:aggr_model_impact_wkt}
\end{table*}


==> tables/wiktionary_by_group.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        \textbf{Metric} &      \begin{tabular}[c]{@{}c@{}}1.  Semantic\\ w/ supertype\end{tabular} &      \begin{tabular}[c]{@{}c@{}}2. Syntactic\\ w/ supertype\end{tabular} &      \begin{tabular}[c]{@{}c@{}}3. Semantic\\ w/o supertype\end{tabular} &      \begin{tabular}[c]{@{}c@{}}4. Syntactic\\ w/o supertype\end{tabular} \\
        \hline
        $z_{diff}~acc.~\uparrow$       & 57.8\% &                      63.3\% &                      \textbf{66.6\%} &                       59.2\% \\ \hline
        $z_{min\_var}~err.~\downarrow$   & \textbf{31.7\%} &                      42.1\% &                      44.9\% &                       43.3\% \\ \hline
        $MIG~\uparrow$                   &  0.091 &                      0.088 &                      0.080 &                       \textbf{0.105} \\ \hline
        $Modularity~\uparrow$            &  0.361 &                      \textbf{0.714} &                      0.424 &                       0.618 \\ \hline
        $Explicitness~\uparrow$          &  0.612 &                      0.566 &                      \textbf{0.638} &                       0.575 \\ \hline
        $Disentanglement Score~\uparrow$ &  0.011 &                      0.015 &                      0.008 &                       \textbf{0.018} \\ \hline
        $Completeness Score~\uparrow$    &  0.011 &                      0.014 &                      0.010 &                       \textbf{0.016} \\ \hline
        $Informativeness Score~\downarrow$ &  0.392 &                      0.429 &                      0.357 &                       \textbf{0.337} \\ \hline
    \end{tabular}

    \caption{Wiktionary dataset - Mean impact of the DSR categorical biases by generative factor grouping.}
    \label{tab:aggr_grouping_impact_wkt}
\end{table*}


==> tables/wordnet_all.tex <==
\begin{table*}[ht!]
    \centering
    \scriptsize
    %\resizebox{.95\columnwidth}{!}
    \begin{tabular}{ll|c|c|c|c|}
\cline{3-6}
                                       & \textbf{}               & \multicolumn{4}{c|}{\textbf{Groupings}}                                                                                                                                                                                                                                               \\ \hline
\multicolumn{1}{|l|}{\textbf{Metrics}} & \textbf{Experiments}    & \begin{tabular}[c]{@{}c@{}}1. Semantic\\ w/ supertype\end{tabular} & \begin{tabular}[c]{@{}c@{}}2. Syntactic\\ w/ supertype\end{tabular} & \begin{tabular}[c]{@{}c@{}}3. Semantic\\ w/o supertype\end{tabular} & \begin{tabular}[c]{@{}c@{}}4. Syntactic\\ w/o supertype\end{tabular} \\ \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & 66.6\% &                      69.9\% &                      69.7\% &                       73.7\%                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$z_{diff}~acc.~\uparrow$}  & 2. Joint DSR loss       & 68.5\% &                      68.2\% &                      69.2\% &                       70.7\%                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & \textbf{77.2\%} &                      \textbf{76.1\%} &                      \textbf{78.9\%} &                       \textbf{75.8\%}                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & \textbf{38.9\%} &                      \textbf{49.9\%} &                      \textbf{47.0\%} &                       \textbf{57.1\%}                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{$z_{min\_var}~err.~\downarrow$} & 2. Joint DSR loss       & 41.0\% &                      52.1\% &                      48.5\% &                       59.5\%                                                                \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & 42.5\% &                      54.6\% &                      51.4\% &                       64.3\%                                                                \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         &\textbf{ 0.074} &                      \textbf{0.068} &                      0.043 &                       \textbf{0.082}                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{$MIG~\uparrow$}              & 2. Joint DSR loss       & 0.065 &                      0.059 &                      0.033 &                       0.070                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & 0.070 &                      0.054 &                      \textbf{0.051} &                       0.061                                                                 \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & 0.737 &                      0.888 &                      0.697 &                       0.851                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{$Modularity~\uparrow$}       & 2. Joint DSR loss       & \textbf{0.745} &                      \textbf{0.900} &                      \textbf{0.705} &                       \textbf{0.866}                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & 0.674 &                      0.880 &                      0.666 &                       0.841                                                                 \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & 0.511 &                      0.511 &                      0.550 &                       0.504                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{$Explicitness~\uparrow$}     & 2. Joint DSR loss       & \textbf{0.522} &                      \textbf{0.528} &                      0.559 &                       \textbf{0.516}                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & 0.521 &                      0.512 &                      \textbf{0.564} &                       0.513                                                                 \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & 0.034 &                      0.020 &                      0.004 &                       0.029                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{$Disentang. Score~\uparrow$} & 2. Joint DSR loss       & 0.034 &                      0.019 &                      0.004 &                       0.027                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & \textbf{0.047} &                      \textbf{0.032} &                      \textbf{0.007} &                       \textbf{0.040}                                                                 \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & 0.022 &                      0.012 &                      0.003 &                       0.014                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{$Completeness~\uparrow$}     & 2. Joint DSR loss       & 0.023 &                      0.012 &                      0.003 &                       0.014                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & \textbf{0.028} &                      \textbf{0.017} &                      \textbf{0.006} &                       \textbf{0.018}                                                                 \\ \hline \hline
\multicolumn{1}{|l|}{}                 & 1. VAE reconst.         & \textbf{0.444} &                      0.405 &                      \textbf{0.285} &                       0.323                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{$Informativeness~\downarrow$}  & 2. Joint DSR loss       & 0.447 &                      \textbf{0.397} &                      0.287 &                       \textbf{0.312}                                                                 \\ \cline{2-6}
\multicolumn{1}{|l|}{}                 & 3. cVAE ($token | DSR$) & 0.485 &                      0.440 &                      0.320 &                       0.350                                                                 \\ \hline
\end{tabular}

    \caption{WordNet dataset - Impact of the DSR categorical biases: reconstruction. The arrow next to each metric indicates the direction of better disentanglement.}
    \label{tab:reconstr_impact_wn}
\end{table*}


==> tables/wordnet_by_exp.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{|l|c|c|c|}
        \hline
        \textbf{Metric} &      1. VAE reconst. &      2. Joint DSR loss &      3. cVAE ($token | DSR$) \\
        \hline
        $z_{diff}~acc.~\uparrow$       & 70.0\% &              69.1\% &                    \textbf{77.0\%} \\ \hline
        $z_{min\_var}~err.~\downarrow$   &  \textbf{48.2\%} &              50.3\% &                    53.2\% \\ \hline
        $MIG~\uparrow$                   &   \textbf{0.067} &              0.057 &                    0.059 \\ \hline
        $Modularity~\uparrow$            &  0.793 &               \textbf{0.804} &                    0.765 \\ \hline
        $Explicitness~\uparrow$          &  0.519 &               \textbf{0.532} &                    0.527 \\ \hline
        $Disentanglement Score~\uparrow$ &  0.022 &              0.021 &                     \textbf{0.031} \\ \hline
        $Completeness Score~\uparrow$    &  0.013 &              0.013 &                     \textbf{0.017} \\ \hline
        $Informativeness Score~\downarrow$ &  0.364 &               \textbf{0.361} &                    0.399 \\ \hline
    \end{tabular}

    \caption{WordNet dataset - Mean impact of the DSR categorical biases by model architecture.}
    \label{tab:aggr_model_impact_wn}
\end{table*}


==> tables/wordnet_by_group.tex <==
\begin{table*}[ht!]
    \centering
    \begin{tabular}{|l|c|c|c|c|}
        \hline
        \textbf{Metric} &      \begin{tabular}[c]{@{}c@{}}1.  Semantic\\ w/ supertype\end{tabular} &      \begin{tabular}[c]{@{}c@{}}2. Syntactic\\ w/ supertype\end{tabular} &      \begin{tabular}[c]{@{}c@{}}3. Semantic\\ w/o supertype\end{tabular} &      \begin{tabular}[c]{@{}c@{}}4. Syntactic\\ w/o supertype\end{tabular} \\
        \hline
        $z_{diff}~acc.~\uparrow$       &      0.702 &                      0.710 &                      0.720 &                       \textbf{0.732} \\ \hline
        $z_{min\_var}~err.~\downarrow$   &    \textbf{0.406} &                      0.520 &                      0.487 &                       0.599 \\ \hline
        $MIG~\uparrow$                   &    0.070 &                      0.061 &                      0.042 &                       \textbf{0.072} \\ \hline
        $Modularity~\uparrow$            &    0.723 &                      \textbf{0.890} &                      0.692 &                       0.854 \\ \hline
        $Explicitness~\uparrow$          &    0.518 &                      0.518 &                      \textbf{0.557} &                       0.511 \\ \hline
        $Disentanglement Score~\uparrow$ &    \textbf{0.037} &                      0.023 &                      0.005 &                       0.031 \\ \hline
        $Completeness Score~\uparrow$    &    \textbf{0.024} &                      0.013 &                      0.004 &                       0.015 \\ \hline
        $Informativeness Score~\downarrow$ &  \textbf{0.456} &                      0.412 &                      0.295 &                       0.326 \\ \hline
    \end{tabular}

    \caption{WordNet dataset - Mean impact of the DSR categorical biases by generative factor grouping.}
    \label{tab:aggr_grouping_impact_wn}
\end{table*}

